LLMs Know What to Drop: Self-Attention Guided KV Cache Eviction for Efficient Long-Context Inference

Efficient long-context inference is critical as large language models (LLMs) adopt context windows of ranging from 128K to 1M tokens. However, the growing key-value (KV) cache and the high computational complexity of attention create significant bottlenecks in memory usage and latency. In this paper, we find that attention in diverse long-context tasks exhibits sparsity, and LLMs implicitly "know" which tokens can be dropped or evicted at the head level after the pre-filling stage. Based on this insight, we propose Self-Attention Guided Eviction~(SAGE-KV), a simple and effective KV eviction cache method for long-context inference. After prefilling, our method performs a one-time top-k selection at both the token and head levels to compress the KV cache, enabling efficient inference with the reduced cache. Evaluations on LongBench and three long-context LLMs (Llama3.1-8B-Instruct-128k, Llama3-8B-Prolong-512k-Instruct, and Qwen2.5-7B-Instruct-128k) show that SAGE-KV maintains accuracy comparable to full attention while significantly improving efficiency. Specifically, SAGE-KV achieves 4x higher memory efficiency with improved accuracy over the static KV cache selection method StreamLLM, and 2x higher memory efficiency with better accuracy than the dynamic KV cache selection method Quest.

==> temp.tex <==
KV Cache memory and latency analysis" based the following content: "\textbf{Memory Challenge}: KV cache memory is the dominant factor, with a memory complexity of $O(2L \times N)$, where $L$ is the number of layers in the LLM and $N$ is the context length. As a result, supporting large batch sizes becomes challenging, leading to reduced concurrency. To enable long-context inference, additional GPUs are required, which further reduces GPU utilization.

\textbf{Inference Speed Bottleneck}: Attention computation dominates the process. The time complexity is $O(L \times N)$ because each newly generated token requires attention to the entire KV (key-value) cache of length $N$. For long-context inference, where $N \gg L$, this overhead becomes significant.

Therefore, reducing the KV cache size can not only support long-context inference and improve concurrency, but also reduce latency during inference.


    \item The top-$p$ index overlaps of adjacent predictions, and first and last token prediction. Let $\mathcal{I}_{p, i}^{l, h}$ be the top-$p$ (e.g., $p$ = 0.99) indexes of the $i$-th token prediction.
    \begin{equation}
        \mathcal{R}_{adj} = \frac{|\mathcal{I}_{p, i}^{l, h} \cap \mathcal{I}_{p, i+1}^{l, h}|}{|\mathcal{I}_{p, i+1}^{l, h}|} \ \text{and} \ \mathcal{R}_{f2l} = \frac{|\mathcal{I}_{p, 1}^{l, h} \cap \mathcal{I}_{p, i+1}^{l, h}|}{|\mathcal{I}_{p, last}^{l, h}|}.
    \end{equation}


% Different heads pay distinct parts of context. The union of top-k and the frequency distribution indicates that nearly all token's information are utlized by LLMs.

% This means that the sparsity is observed at head-level. The union of top-k indexes at with-in layer and cross-layer is definitely not sparse. 

% The head-level sparsity indicates each head of LLMs has ability to prune the context. Given context and query, it is reasonable to assume that LLMs knows what can be evict or compressed in head-level. Therefore, we make use the attention scores of the last token in the concat of context and query to compress the KV cache in head-level, we only select size $k$ KV cache for each head to guide the token generation. Fig.~\ref{fig:topkIdx_analysis} (d) which selects the top-1024 KV cache for each head to guide the generation on six long-bench tasks, show competive performance to full-kv cache, indicates  the effectiveness of this assumption. This confirms the assumption that LLMs know what to drop or evict once they complete the pre-filling. Based on observation, we design a simple but quite effective method for long context inference, that is, we let LLM itself to compress the KV cache after prefilling and then make use the compressed KV cache to speedup generation. 

% Based on the above analysis, we assume that for long context inference, one-time token-level sparsity is enough. In other words, LLMs know what to drop or evict once they complete the pre-filling.

% Conclusion: 1) Sink, Local is important; 2) nearly all KV indexes are appear. 3) Top-k indexes is head-level, group-query attention show less overlap top-k indexes.

 where $\mathbf{k}_i^{l} \in \mathcal{R}^{h_{kv}\times d_h}$ and $\mathbf{v}_i^{l} \in \mathcal{R}^{h_{kv}\times d_h}$, $h_{kv}$ denotes the KV cache head number and $d_h$ is the head dimension


 These baselines allow for a robust comparison, highlighting the strengths of our proposed approach.

 In this paper, we address the challenges of efficient long-context inference in LLMs by proposing a novel approach based on the observation that LLMs inherently know what to drop once the pre-filling stage is complete. Through extensive and comprehensive analysis, we demonstrate that attention scores can be effectively utilized to guide the compression of the context KV cache. We introduce this algorithm as Self-Attention Guided Eviction (SAGE).

 1. Larger sink size
2. Larger local window size
3. Top-k window size.


Due to the group query attention, for the same memory budget, the reduced KV cache length of the proposed method is shorter than that of StreamLLM. Let $B$ be the memory budget, for StreamLLM the KV cache size is $B$. And for our proposed method, we can divide the budget into three part, sink cache with size $S$, top-$k$ cache and recent or local cache with size $R$. Let $G$ be the group size of group query attention, $B$ = $S + G \times k + R$ and the reduced KV cache size of our method is will $S + k + R < B$ since $G > 1$. Therefore, with the same memory budget, our inference speed will faster than StreamLLM while keeping the comparable performance to full attention. Our speedup ratio comparing to StreamLLM is $\frac{S + k \times G + R}{S + k + R} = 1 + \frac{1}{\frac{B}{(G-1) \times k} - 1}$. Based on our experimental study, it is better to set $S = B/4$, $k \times G = B/2$. Therefore, the speedup ratio comparing to StreamLLM for Llamma3.1-8B-Instruct is $B / (B/4 + B/(2G) + B/4) = 1.6$ since $G = 4$. 

Let $N$ be the the input context length, and $B$ is the memory budget. The attention computation speedup ratio of StreamLLM is $\frac{N}{B}$, and the speedup ratio of our proposed method is $1.6\frac{N}{B}$.

To comprehensively evaluate the performance and robustness of our proposed method, we perform a detailed hyperparameter analysis over eight diverse long-context learning tasks (including QA, summary, code rep, retrieval) of Longbench~\footnote{These tasks consists of six ones used in Quest~\cite{tangquest} for hyper-parameter analysis and two new added ones. They are ''gov-report", ''multifieldqa-en", ''narrativeqa", ''passage-retrieval-en", ''qasper", ''repobench-p", ''hotpotqa" and ''triviaqa".} using Llama3.1-8B-Instruct. The analysis focuses on three key hyper-parameters: memory budget, sink window size, and top-$k$, aiming to understand their impact on accuracy.

Potential explanation: Why once selection is enough: 1) top-k indexes distribution; 2) adjacent top-k overlap; 3) Token-level retrieval show only small top-k (such as 256) is enough~\cite{liu2024retrievalattention}, we set larger top-k (However, we do not need construct complex index as well as only one-time selection with competive performance.

Token-level top-k selection for only once. (For most long context inference tasks, the generated text is short. We can perform one-time top-k selection and share the top-k indexes for continuous generation.

We set the token budget $B$ as 0.5k, 1k, 2k, 4k and 8k, respectively, and collect the average accuracy over eight Longbench tasks with Llama3.1-8B-Instruct with respect to different KV cache eviction methods. Fig.~\ref{fig:hyper_analysis}(a) shows the impact of token budget $B$ over the average accuracy. From this figure, we observe that: 1) with the increase the token budget, the performance of all methods increases; 2) the performance of our method \name is significantly higher than the static sparse pattern based StreamLLMs under all token budgets. Since StreamLLM directly discards the middle parts of input sequence. This indicates the importance of one-time top-k token selection since with same budget, since our method \name is always better than StreamLLM. 3) The performance of our method \name under 2k is close to the performance of StreamLLM under 8k. This means that our method is around 4x memory efficient comparing to StreamLLM over Longbench with Llama3.1-8B-Instruct.

We evaluate the impact of sink window size on our method and StreamLLM by given a fixed token budget $B$ = 8192. For our method \name, we set the top-$k$ as 1024. By setting sink window size $S$ as 8, 32, 128, 512, 1024, 2048, 3072, 3584, we collect the average accuracy across eight Longbench tasks using Llama3.1-8B-Instruct with different KV cache eviction methods. Fig.~\ref{fig:hyper_analysis} (b) shows the impact of sink window size on the average accuracy. From this figure, we observe that: with the increase of sink window size, the performance of all StreamLLM increases. Our method \name increase a little when $S$ is very large. This indicates that our method is more robust to the sink window size since our method can recover the important tokens appearing in the starting of input by top-$k$ selection. StreamLLM needs to increase the sink window size if there are important tokens at the beginging of the input.


To explore the impact top-$k$ of \name on long context learning with Llama3.1-8B-Instruct. We set the token budget $B$ as 8192 and sink window size as $B/4$ = 2048 according to sink window size analysis above, and vary $k$ as 8, 64, 128, 256, 512 and 1024 and collect the average accuracy across eight Longbench tasks. Fig.~\ref{fig:hyper_analysis} (c) shows the impact of $k$ on the accuracy. From this figure, we observe that, with the increase of $k$, the performance of \name increases at first and then drops. This means larger $k$ increase the chance to find more important tokens in middle of input sequence. According to the attention analysis in Fig.~\ref{fig:topkIdx_analysis} (c), the ratio of important tokens in middle of input is non-negligible. 

However, with the increase of $k$, the accuracy drops. This can be explained as that, given fixed token budget, increase of $k$ means that the recent window size is small, since the local window size $R$ = $B - S - G\times k$ since we select top-$k$ for each query head and $G$ is the query group number. Smaller $R$ results in we might miss some important recent tokens not in recent window but top-$k$ missed. Moreover, the drop ratio is only 0.4\% from the highest to lowest, this means that \name is still robust to top-k. In practice, given budget $B$ and LLM with query group number $G$, the suggest $k$ of \name is between $\frac{B}{4G}$ and $\frac{B}{2G}$.


In contrast, dynamic sparsity methods, adaptively select representative tokens for each new token generation. While these methods typically achieve better performance compared to static sparsity approaches, they are more computationally intensive and depend on carefully tuned hyperparameters, such as the chunk size in InfLLM~\cite{xiao2024infllm} and Quest~\cite{tangquest}, and Retrieval Attention~\cite{liu2024retrievalattention} needs to construct complex graph-based indices to efficiently identify representative tokens for each new token generation. These dynamic methods do not mitigate the memory footprint since they need to save all the KV cache as candidate for selection at each generation step. A naive solution based on sparse attention involves offloading the KV cache to the CPU to reduce memory usage. Nonetheless, this approach incurs significant overhead due to the latency of fetching the selected sparse KV pairs from the CPU during decoding. Therefore, dynamic methods often require intricate designs to balance computational efficiency and communication overhead. They typically involve tightly coordinated CPU-GPU computations or communication mechanisms to achieve the desired efficiency, which adds implementation complexity~\cite{xiao2024infllm}.


Efficient long-context inference is essential as large language models (LLMs) adopt context windows up to 128K or 1M tokens. However, the expanding key-value (KV) cache and the high computational complexity of attention severely hinder inference throughput, making memory usage and latency critical bottlenecks. In this paper, by extensive attention distribution analysis over diverse long context inference tasks. We observe and assume that LLMs know what to drop or evict once they complete the pre-filling over given context and query. We propose a simple and effective KV eviction method, Self-attention Guided Eviction of KV cache (\name),  for long-context inference. Specifically, after the prefilling stage, a one-time top-$k$ selection is performed at both the token and head levels to compress the KV cache. The model then utilizes this compressed KV cache for inference. Our evaluation over two well-known benchmarks (LongBench and InfiniteBench) and three long context LLMs (Llama3.1-8B-Instruct, Llama3-8B-Prolong-512k-Instruct and Qwen2.5-Instruct) demonstrates that our method delivers accuracy comparable to full attention and other dynamic KV selection methods but with noticeably better efficiency, our efficiency approach to the static sparse pattern based method StreamLLM. Moreover, our method demonstrates superior memory efficiency (4x) compared to StreamLLM, while also achieving a significant improvement in accuracy.

The efficiency of LLMs during inference is significantly constrained by memory usage and latency, particularly in long-context scenarios. This section explores the challenges posed by the KV (Key-Value) cache and its impact on both memory consumption and inference speed.

KV cache memory is a major factor contributing to high memory consumption during inference. Its memory complexity is $O(2L \times N)$, where $L$ is the number of layers and $N$ denotes the context length (number of tokens in the input). As the context length increases, the memory demands grow significantly, making it difficult to support large batch sizes and reducing the ability to process multiple requests simultaneously (concurrency) (see Fig.~\ref{fig:memory_length} (a) and (b)). The handling of longer contexts often requires additional GPUs, which further reduces overall GPU utilization and efficiency.

Inference speed is also heavily impacted by the attention mechanism. From Fig.~\ref{fig:memory_length} (c), the latency of single token generation is dominated by attention computation for long context inference. Each newly generated token requires attending to the entire KV cache of length $N$, resulting in a time complexity of $O(L \times N \times d^2)$, where $d$ is the hidden size. The time complexity of feed-forward networks (e.g., $d \times 3.5d \times d$ for Llama-3.1-8B-Instruct) for a single token generation is $O(7L\times d^2)$. In long-context scenarios where $N \gg 7$, this repeated computation becomes a significant bottleneck, slowing down the generation process.


In this paper, we tackle the challenges of efficient long-context inference in LLMs by leveraging the observation that LLMs inherently possess the ability to identify the critical information after the pre-filling stage. Through a comprehensive analysis of attention scores across well-known long-context learning benchmarks (See details in Sec.~\ref{subsec: attn}), we demonstrate that attention scores exhibit head-level sparsity and effectively highlight the importance of tokens within the context.  Our analysis reveals that attention scores, which show head-level sparsity and reflect the importance of tokens in the context, can serve as a reliable basis for optimizing the compression of the context KV cache in head-level. Building on this insight, we propose a novel KV cache compression method called \textbf{Self-Attention Guided Eviction of KV cache} (\name), which utilizes attention scores to guide the eviction process and improve the efficiency of long-context inference.


Our method \name introduces a single-pass head-level dynamic selection strategy, where a one-time compression of the KV cache is performed after the prefilling stage (Please refer to Fig.~\ref{fig:framework} in Sec.~\ref{sec: method} for details). This eliminates the need for repetitive computations during token generation, significantly reducing computational overhead. The resulting compressed KV cache retains the most relevant information, enabling efficient and accurate inference. Our approach combines the efficiency of static patterns with the adaptability of dynamic methods, achieving superior efficiency while maintaining competitive or even better performance compared to existing dynamic approaches based on our extensive experimental stduy over different long context LLMs and benchmarks. 


We believe that this method represents a simple yet highly effective solution for accelerating long-context inference. Its combination of simplicity, effectiveness, and ease of integration offers a promising direction for addressing the challenges of long-context LLM inference.


This section first explores the challenges of LLM inference in long context scenarios since LLM inference efficiency is heavily limited by memory usage and latency, especially in long-context scenarios, and get the conclusion that KV cache optimization is quite critical and important for effecient inference. 

Afterwards, we do a comprehensive attention score analysis to explore effective KV cache compression techniques, and find the attention sparsity is general for long context inference,  attention sparsity is is head-level and attention scores are a good metrics for KV cache eviction, and this plays a fundation to  our proposed method.


We select the Llama-3.1-8B-Instruct model as the backbone LLM for a comprehensive analysis of attention over LongBench~\citep{bai2023longbench} and InfiniteBench~\citep{zhang2024bench}. Specifically, for each task in these two benchmarks, we randomly select five examples and collect attention scores from every head and layer of the LLM. This is done for both the first token generation and token generation at another specified position.

Let $L$ and $H$ be the number of layers of LLM, the head number of attention heads per layer, respectively. Suppose that $N$ is the sequence length or KV cache size, and $k$ ($k \leq N$) is the number of top attention scores to retrain per head. Then the attention scores for a given layer $l$ ($1\leq l \leq L$) and head $h$ ($1\leq h \leq H$) can be represented as:
\begin{equation}\label{eq:attention_score}
    \mathbf{S}^{l, h} = [s_{1}^{l,h}, s_{2}^{l,h}, \cdots, s_{N}^{l,h}] \land \sum_{i=1}^{N}s_{i}^{l,h} = 1.
\end{equation}

Then, we compute top-$k$ attentions scores $\mathbf{S}_{k}^{l,h}$ and $\mathcal{I}_{k}^{l,h}$ indexes as follows:
\begin{equation}\label{eq:topk_score}
        \mathbf{S}_{k}^{l,h} = \{s_{i}^{l,h} | i \in \mathcal{I}_{k}^{l,h}\}, \ \text{and} \  \mathcal{I}_{k}^{l,h} = \{i_1, i_2, \cdots, i_k|s_{i_1} \leq s_{i_2} \cdots \leq s_{i_k}, i_j \in \{1, 2, \cdots, N\}\}
\end{equation}

We also collect the top-$p$ token indexes (e.g., $p$ = 0.99). Let $\mathcal{I}^{l,h} = \text{argsort}_{{\text{desc}}}(\mathbf{S}^{l, h})$ represent the indices of the attention score $\mathbf{S}^{l, h}$ ordered in descending order. Then, we get the top-$p$ indexes by:
\begin{equation}
    \mathcal{I}_{p}^{l,h} = \{ i \mid i \in \mathcal{I}^{l,h}[:k], k = \min \{k^{\prime}\mid \sum_{j\in \mathcal{I}[:k^{\prime}]} s_{j}^{l, h} \geq p\} \}
\end{equation}
Memory and latency analysis of Llama3-8B-ProLong-512k across different context lengths: (a) and (b) show that KV cache dominates memory usage during long-context inference, while (c) reveals that attention computation is the primary contributor to latency when generating a new token in long-context scenarios.

This section first explores the challenges of LLM inference in long-context scenarios, focusing on how memory usage and latency limit efficiency. We conclude that optimizing the KV cache is critical for achieving efficient inference.

Next, we perform a comprehensive analysis of attention scores to investigate effective KV cache compression techniques. Our findings reveal that attention sparsity is prevalent in long-context inference, operates at the head level, and that attention scores serve as an effective metric for KV cache eviction, forming the foundation of our proposed method.

\xhdr{Top-$k$ Attention Score Analysis} We compute the sum of top-$k$ attention scores per head $sum_{k}^{l,h} = \sum_{i=1}^{k}\mathbf{S}_{k}^{l,h}[i]$. Then, we can get $L\times H$ sum of top-$k$ attention scores, and draw heat-map of these $L\times H$ scores. 

We calculate the sum of the top-k attention scores from multiple examples drawn from diverse tasks on LongBench and InfiniteBench. All selected examples have input lengths of at least 16k tokens. The attention scores are gathered for two specific scenarios: the generation of the first token and the generation of a token at a specified position. Afterwards, we visualize the attention distribution by the following methods:
\begin{itemize}[leftmargin=2pt]
    \item \textbf{Heatmap}: A heatmap is generated for each example, where rows represent the layer index and columns represent the head index. Darker shades correspond to higher sums of the top-k attention scores.
    
    \item \textbf{Boxplot} For each layer, the sum of the top-k attention scores is aggregated across all examples. The aggregated distribution is visualized using a boxplot to show statistical summaries.

    \item \textbf{Pie Chart} The sum of the top-$k$ attention scores across all layers and examples is combined to generate a pie chart. The scores are grouped into intervals: $(0, 0.5]$, $(0.5, 0.8]$, and $(0.8, 0.9]$ and $(0.9, 1]$.
\end{itemize}


We compute the sum of top-$k$ attention scores per head $sum_{k}^{l,h} = \sum_{i=1}^{k}\mathbf{S}_{k}^{l,h}[i]$. Then, we can get $L\times H$ sum of top-$k$ attention scores, and draw heat-map of these $L\times H$ scores. 

We calculate the sum of the top-k attention scores from multiple examples drawn from diverse tasks on LongBench and InfiniteBench. All selected examples have input lengths of at least 16k tokens. The attention scores are gathered for two specific scenarios: the generation of the first token and the generation of a token at a specified position. Afterwards, we visualize the attention distribution by the following methods:
\begin{itemize}[leftmargin=2pt]
    \item \textbf{Heatmap}: A heatmap is generated for each example, where rows represent the layer index and columns represent the head index. Darker shades correspond to higher sums of the top-k attention scores.
    
    \item \textbf{Boxplot} For each layer, the sum of the top-k attention scores is aggregated across all examples. The aggregated distribution is visualized using a boxplot to show statistical summaries.

    \item \textbf{Pie Chart} The sum of the top-$k$ attention scores across all layers and examples is combined to generate a pie chart. The scores are grouped into intervals: $(0, 0.5]$, $(0.5, 0.8]$, and $(0.8, 0.9]$ and $(0.9, 1]$.
\end{itemize}

We collect the following metrics to investigate the distribution of the top $k$ indexes.

\begin{enumerate}[leftmargin=4pt, label=(\arabic*)]
    \item \textbf{Within layer metrics}, the Jaccard similarity of top-$k$ indexes of $H$ heads, and the coverage ratio of the union of the top-$k$ indexes $\mathcal{U}_{k}^{l} = \bigcup_{i=1}^{H}\mathcal{I}_{k}^{l, i}$ to the entire context length.
    \begin{equation}
        \mathcal{J}^{l} = \frac{|\bigcap_{i=1}^{H}\mathcal{I}_{k}^{l, i}|}{|\bigcup_{i=1}^{H}\mathcal{I}_{p}^{l, i}|}, \ \text{and} \ \mathcal{R}_{c}^{l} = \frac{|\mathcal{U}_{k}^{l}|}{N},
    \end{equation}
    where $|X|$ represents the number of elements in $X$. $\mathcal{J}^{l}$ indicates the overlap ratio of top-$k$ indexes of $H$ heads in layer $l$. $\mathcal{R}_{c}^{l}$ indicates the ratio of tokens being effective or triggered by top-$k$ selection for inference in layer $l$.
    
    \item \textbf{Cross all-layer metrics}, Jaccard similarity of union of top-$k$ indexes $\mathcal{U}_{k}^{l}$ cross all $L$ layers, and the coverage ratio of the union of all union top-$k$ indexes of all layers to the entire context length.
    \begin{equation}
        \mathcal{J} = \frac{|\bigcap_{i=1}^{L}\mathcal{U}_{k}^{i}|}{|\bigcup_{i=1}^{L}\mathcal{U}_{k}^{i}|} \ \text{and} \ \mathcal{R}_{c} = \frac{|\bigcup_{i=1}^{L}\mathcal{U}_{k}^{i}|}{N}
    \end{equation}
    $\mathcal{J}$ indicates the ratio of top-$k$ tokens shared by $L$ layers. $\mathcal{R}_{c}$ indicates the ratio of tokens being effective or triggered by top-$k$ selection for inference.
    
    \item Token index frequency distribution of the top-$p$ indices across all heads and all layers. For $i$-th token ($0\leq i \leq N$), its frequency is defined as: 
    \begin{equation}
        \text{freq}_{i} = \frac{\sum_{l=1}^{L}\sum_{h=1}^{H} \mathbf{1}_{ i \in \mathcal{I}_{p}^{l, h}}}{L \times H}.
    \end{equation}
\end{enumerate}

Analysis of top-$k$ index distribution for Llama3.1-8B-Instruct. (a) Within-layer Jaccard similarity $\mathcal{J}^{l}$  of $H$ top-4096 indexes and coverage ratio $\mathcal{R}{c}^{l}$ based on 165 examples for first token generation. (b) Cross-layer intersection ratio $\mathcal{R}$ and coverage ratio $\mathcal{R}{c}$ collected from 165 examples, sorted by context length. The light blue line represents the normalized context length, calculated as input length divided by 128k. (c) Top-$p$ ($p$ = 0.975) token index frequency distribution for a NarrativeQA example with a context length of 64k tokens. (d) Performance of once Top-1000 KV Cache eviction vs. Full KV cache over six longbench tasks.

We show the attention score distribution results from two aspects: top-k attention score distribution and top-k/p index distribuion. Based on the distribution analysis, we find that sparsity of the attention scores is general accross different tasks, and the sparsity is head-level, as well as we observe that attention scores are effective metrics to compress KV cache, and further design a simple but quite efficient KV cache eviction method for fast long context inferece. We just show the observation in this section, the detailed analysis method and experimental settings can be found in appendix.
\begin{figure}[h!]
    \centering
    % First subfigure
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/within_layer_topk.pdf}
        \caption{Within-Layer Metric}
        \label{fig:sub1}
    \end{subfigure}
    % Second subfigure
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/cross_layer_topk.pdf}
        \caption{Cross-Layer Metric}
        \label{fig:sub2}
    \end{subfigure}
    % Third subfigure
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/top_index_freq.pdf}
        \caption{Index frequency}
        \label{fig:sub3}
    \end{subfigure}
    % Third subfigure
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/performance_example.pdf}
        \caption{Acc Comp.}
        \label{fig:sub3}
    \end{subfigure}    
    % Caption for the main figure
    \caption{Analysis of top-$k$ index distribution for Llama3.1-8B-Instruct. (a) Within-layer Jaccard similarity of top-4096 indexes and coverage ratio based on 165 examples for first token generation. (b) Cross-layer intersection ratio and coverage ratio collected from 165 examples, sorted by context length. The light blue line represents the normalized context length, calculated as input length divided by 128k. (c) Top-$p$ ($p$ = 0.975) token index frequency distribution for a NarrativeQA example with a context length of 64k tokens. (d) Performance of once Top-1000 KV Cache eviction vs. Full KV cache over six longbench tasks.}
    \label{fig:topkIdx_analysis}
\end{figure}


\begin{figure}[h!]
    \centering
    % First subfigure
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/within_layer_topk.pdf}
        \caption{Within-Layer Metric}
        \label{fig:sub1}
    \end{subfigure}
    % Second subfigure
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/cross_layer_topk.pdf}
        \caption{Cross-Layer Metric}
        \label{fig:sub2}
    \end{subfigure}
    % Third subfigure
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/top_index_freq.pdf}
        \caption{Index frequency}
        \label{fig:sub3}
    \end{subfigure}
    % Third subfigure
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/performance_example.pdf}
        \caption{Acc Comp.}
        \label{fig:sub3}
    \end{subfigure}    
    % Caption for the main figure
    \caption{Analysis of top-$k$ index distribution for Llama3.1-8B-Instruct. (a) Within-layer Jaccard similarity $\mathcal{J}^{l}$  of $H$ top-4096 indexes and coverage ratio $\mathcal{R}{c}^{l}$ based on 165 examples for first token generation. (b) Cross-layer intersection ratio $\mathcal{R}$ and coverage ratio $\mathcal{R}{c}$ collected from 165 examples, sorted by context length. The light blue line represents the normalized context length, calculated as input length divided by 128k. (c) Top-$p$ ($p$ = 0.975) token index frequency distribution for a NarrativeQA example with a context length of 64k tokens. (d) Performance of once Top-1000 KV Cache eviction vs. Full KV cache over six longbench tasks.}
    \label{fig:topkIdx_analysis}
\end{figure}

Fig.~\ref{fig:topkIdx_analysis} of attention distribution analysis reveals that sparsity in attention is observed at the head-level (Fig.~\ref{fig:attn_heatmap} (a)), rather than at the layer-level or across all layers. Each attention head focuses on distinct parts of the context, as evidenced by the union of top-$k$ indexes and their frequency distribution, which show that nearly all token information is utilized by LLMs. However, the union of top-$k$ indexes within a single layer or across multiple layers is not sparse (see Fig~\ref{fig:topkIdx_analysis} (a), (b) and (c)), confirming that sparsity is specific to the head-level.

This head-level sparsity suggests that each attention head in an LLM has the ability to prune the context. Given a context and a query, it is reasonable to assume that LLMs can identify which information to evict or compress at the head-level. Leveraging this insight, we use the attention scores of the last token in the concatenated context and query to compress the KV cache at the head-level. Specifically, we select a KV cache of size $k$ for each head to guide token generation.

As shown in Fig.~\ref{fig:topkIdx_analysis}(d), selecting the top-1024 KV cache for each head achieves competitive performance compared to using the full KV cache on six LongBench tasks. This confirms our assumption that LLMs inherently know what to retain and what to discard after the pre-filling stage.

Attention score analysis of Llama3.1-8B-Instruct. (a) Heatmap showing the sum of the top 4096 attention scores for the first token generation in a NarrativeQA example with a context length of 64k tokens. (b) Boxplot illustrating the distribution of the sum of attention scores for the first token generation across all layers, based on 165 examples from LongBench and InfiniteBench with context lengths $\geq$ 16k (a similar distribution is observed for non-initial token generations). (c) Pie chart depicting the distribution of the sum of attention scores across all layers for non-initial token generations in the same 165 examples (a similar distribution is observed for first token generations).

Analysis of top-$k$ index distribution for Llama3.1-8B-Instruct. (a) Within-layer Jaccard similarity of top-4096 indexes and coverage ratio based on 165 examples for first token generation. (b) Cross-layer intersection ratio and coverage ratio collected from 165 examples, sorted by context length. The light blue line represents the normalized context length, calculated as input length divided by 128k. (c) Top-$p$ ($p$ = 0.975) token index frequency distribution for a NarrativeQA example with a context length of 64k tokens. (d) Performance of Top-1k selection based KV Cache eviction vs. Full KV cache over six longbench tasks.

 SAGE significantly improves efficiency while maintaining strong performance, offering a practical solution for long-context inference.

 \xhdr{Top-$k$ selection} When attention scores for the last token are available, top-k selection has a time complexity of $O(E \log E)$, where $E$ is the size of the KV cache marked for eviction. For methods like FlashAttention~\citep{dao2022flashattention} that do not return attention scores, top-$k$ can be computed using the dot product between the last token query vector and the evicted key cache, with a time complexity of $O(E \times d + E \log E)$, which simplifies to $O(E \times d)$ since $d \gg \log E$ in practice.

To minimize the impact on Time-to-First Token (TTFT), pipeline parallelism can be employed, allowing top-$k$ selection for layer $l-1$ to run concurrently with the self-attention computation of layer $l$. This ensures TTFT remains unaffected, even without attention scores. Furthermore, dot-product-based top-k selection eliminates the softmax overhead, enabling faster execution and parallel computation of scores for improved efficiency.

\xhdr{Top-$k$ selection} When attention scores for the last token are available, top-k selection has a time complexity of $O(E \log E)$, where $E$ is the size of the KV cache marked for eviction. For methods like FlashAttention~\citep{dao2022flashattention} that do not return attention scores, top-$k$ can be computed using the dot product between the last token query vector and the evicted key cache, with a time complexity of $O(E \times d + E \log E)$, which simplifies to $O(E \times d)$ since $d \gg \log E$ in practice.

To minimize the impact on Time-to-First Token (TTFT), pipeline parallelism can be employed, allowing top-$k$ selection for layer $l-1$ to run concurrently with the self-attention computation of layer $l$. This ensures TTFT remains unaffected, even without attention scores. Furthermore, dot-product-based top-k selection eliminates the softmax overhead, enabling faster execution and parallel computation of scores for improved efficiency.


For methods like FlashAttention~\citep{dao2022flashattention} that do not return attention scores, top-$k$ can be computed using the dot product between the last token query vector and the evicted key cache, with a time complexity of $O(E \times d + E \log E)$, which simplifies to $O(E \times d)$ since $d \gg \log E$ in practice.

, even without attention scores. Furthermore, dot-product-based top-k selection eliminates the softmax overhead, enabling faster execution and parallel computation of scores for improved efficiency

To further minimize the impact on Time-to-First Token (TTFT), pipeline parallelism can be employed, allowing top-$k$ selection for layer $l-1$ to run concurrently with the self-attention computation of layer $l$. This ensures TTFT remains unaffected.

Comparing to dynamic chunk-wise top-k selection, such as Quest and InfLLM, for single token generation, the time complexity is $O(L\times \frac{N}{C}\times d)$ for critical block score computation and $O(L\times \frac{N}{C}\log (\frac{N}{C})$ for top-$k$ block selection, where $C$ represents the chunk-size. Suppose $T$ tokens are generated, the total time complexity of Quest is $O(L\times T\times \frac{N}{C}\times(d +\log (\frac{N}{C})))$. In practice, $C$ is usually set the value being less than 16 to get a tradeoff between accuracy and latency, $E < N$ and $\log E < T\times \frac{d}{C}$. Therefore, top-$k$ selection of \name is more efficient than that of dynamic top-$k$ selection.


2) Our method, \name, consistently outperforms the static sparse pattern-based StreamLLMs across all token budgets. This is because StreamLLM discards the middle sections of the input sequence, resulting in significant information loss. In contrast, \name uses a one-time top-$k$ token selection strategy, which is more effective within the same budget. This indicates the contribution of our proposed self-attention guided KV evication. 3) The performance of \name with a 2k token budget is comparable to that of StreamLLM with an 8k token budget. This indicates that \name is approximately 4× more memory efficient than StreamLLM on Longbench tasks with Llama3.1-8B-Instruct. These findings highlight the importance of our proposed attention-guided KV eviction method, as it enables better performance while significantly reducing memory usage. 4) The performance of \name with a 4k token budget is comparable to that of Quest with an 8k token budget. This indicates that \name is approximately 2× more memory efficient than Quest on Longbench tasks with Llama3.1-8B-Instruct. Quest identifies that important tokens based on chunk-representation which results in in-accuracte top-k results. \name performs top-k selection in the token-level and thus results in more accurate context detection and further better results. This confirms that LLMs knows what to drop

1) As the token budget increases, the performance of all methods improves. This demonstrates that larger token budgets allow for better information retention and higher accuracy. 2) \name consistently outperforms the static sparse pattern-based StreamLLMs across all token budgets by avoiding the significant information loss caused by StreamLLM’s removal of middle sections in the input sequence. Instead, \name employs a one-time top-$k$ token selection strategy, effectively preserving critical information within the same budget. This demonstrates the effectiveness of our self-attention-guided KV eviction method. 3) With a 2k token budget, \name achieves comparable performance to StreamLLM with an 8k token budget, demonstrating approximately 4× higher memory efficiency on LongBench tasks with Llama3.1-8B-Instruct. These results highlight how attention-guided KV eviction significantly improves performance while reducing memory usage. 4) \name with a 4k token budget matches Quest’s performance at an 8k token budget, offering 2× higher memory efficiency. Unlike Quest, which relies on less accurate chunk-level representations for top-$k$ selection, \name performs token-level selection, enabling more precise context detection and better results. This confirms that LLMs inherently identify which tokens to retain or discard.


This section presents the attention score distribution analysis from two perspectives: top-$k$ attention score distribution and top-$k$/$p$ index distribution. Our findings reveal that attention score sparsity is a common phenomenon across tasks, primarily at the head level. Moreover, attention scores prove to be effective metrics for KV cache compression, forming the basis of our efficient KV cache eviction method for fast long-context inference. Detailed analysis methods and experimental settings are provided in the appendix.


\textbf{The illustration of \name with the single-pass KV cache selection process}. The full KV cache is divided into four components: initial tokens, tokens designated for eviction, recent tokens, and the last token. To construct the final KV cache, the top-$k$ tokens are selected based on the attention scores between the last token and the tokens marked for eviction at the head level. The final KV cache is formed by concatenating the initial tokens, the selected top-k tokens, and the recent tokens. This updated cache is used for continuous token generation. When a new token (shown in green) is generated, it is added to the recent tokens, updating the recent window for the next step generation.

By leveraging group query attention, \name reduces the KV cache size while maintaining the same token budget $B$. This can be explained as follow. 

First, the KV cache size is $B$ for StreamLLM if token budget is $B$.


In comparison, our method \name divide $B$ KV Cache into three components: the sink cache ($S$), top-$k$ cache ($k \times G$, where $G$ is the group size of group query attention), and recent cache ($R$). Thus, $B = S + G \times k + R$. Since $G > 1$, the effective KV cache size in our method becomes $S + k + R < B$, allowing for faster inference while maintaining performance comparable to full attention. 

We present \name, an efficient KV cache eviction method for long-context LLM inference. Leveraging the inherent attention sparsity of LLMs, which enables them to identify critical context and further compress the KV Cache, \name uses attention scores to reduce the KV cache after the prefilling stage. This compressed cache is then used directly for generation. Empirical experiments demonstrate that \name maintains competitive accuracy relative to full attention while achieving inference speeds comparable to static sparse methods. Notably, \name achieves 4× higher memory efficiency and significant improved accuracy compared to the static sparse method StreamLLM, and 2× higher memory efficiency with better accuracy than the dynamic sparse method Quest. Furthermore, \name is fully compatible with existing LLM frameworks, including Hugging Face Transformers, Meta’s LLaMA, and Alibaba’s Qwen, allowing for seamless integration into existing pipelines.

We analyze the impact of sink window size $S$  on our method (\name) and StreamLLM, using a fixed token budget $B$ = 8192. For \name, we set top-$k$  to 1024. We evaluate the average accuracy across eight Longbench tasks using Llama3.1-8B-Instruct with different KV cache eviction strategies, varying $S$ as 8, 32, 128, 512, 1024, 2048, 3072, and 3584. 

The results are shown in Fig.~\ref{fig:hyper_analysis} (b). From the figure, we observe that the performance of all StreamLLM methods improves as $S$ increases. In comparison, the performance of \name shows only slight improvement when $S$  becomes very large. This demonstrates that \name is more robust to sink window size, as it effectively recovers important tokens from the beginning of the input through top-$k$ selection. In contrast, StreamLLM relies more heavily on increasing $S$  to account for important tokens at the start of the input. In practice, the suggested sink window size under given token budget $B$ is between $\frac{B}{8}$ and $\frac{B}{4}$.


From this figure, we observe that: with increasing $k$ initially improves performance but eventually leads to a decline. Larger $k$ values enhance the ability to capture more important tokens from the middle of the input sequence, as shown in the attention distribution analysis in Fig.\ref{fig:topkIdx_analysis}(c), where the middle tokens contribute a non-negligible portion of the attention. 

However, as $k$ increases further, accuracy decreases. This is because, given a fixed token budget, larger $k$ reduces the size of the recent window $R$, calculated as $R = B - S - G \times k$, where $G$ is the query group number, and $S$ is the sink window size. A smaller $R$ increases the likelihood of missing important recent tokens that fall outside the recent window or are not selected as part of the top-$k$.


Despite this, the performance drop is marginal—only 0.4\% from the highest to the lowest accuracy—indicating that \name remains robust to variations in $k$. In practice, for a token budget $B$ and a query group number $G$ of the LLM, we recommend setting $k$ within the range $\frac{B}{4G}$ to $\frac{B}{2G}$ for optimal performance.

By combining the efficiency of static sparse patterns (single-pass and keep fixed in following generation) with the adaptability of dynamic selection methods (KV cache selection is context related), \name achieves superior efficiency while providing competitive or better performance compared to existing dynamic approaches, as demonstrated in our extensive experiments across various long-context LLMs and benchmarks.

our implementation of StreamLLM demonstrates significantly better performance compared to the HuggingFace (HF) official implementation with Qwen2.5-7B-Instruction and slightly better average accuracy with Llama3.1-8B-Instruct. This improvement is likely due to a flaw in the HF implementation, where the RoPE rotation operation for converting key cache positions to relative positions within the token window fails to account for the latest token, resulting in disproportionately large relative distances for adjacent tokens. This issue, documented in Hugging Face Issue\footnote{\url{https://github.com/huggingface/transformers/issues/35350}}, appears to particularly affect Qwen2.5’s sensitivity to positional encoding. In contrast, our implementation ensures that the relative distance between adjacent tokens remains smaller than that of distant tokens, yielding more consistent results. This highlights the importance of careful implementation when comparing StreamingLLM, especially for tasks and models sensitive to token-relative distances


We set the token budget $B$ = 8192 and the sink window size to $B$/4 = 2048 (based on sink window analysis). We varied $k$ as 8, 64, 128, 256, 512, and 1024, measuring the average accuracy across eight LongBench tasks (Fig.~\ref{fig:hyper_analysis}(c)). Initially, increasing $k$ improves performance by capturing more important tokens from the middle of the input sequence, as indicated in Fig.~\ref{fig:topkIdx_analysis}(c), where middle tokens contribute significantly to attention. However, as $k$ increases further, accuracy declines due to a reduction in the recent window size $R = B - S - G \times k$, where $G$ is the query group number and $S$ is the sink window size. A smaller $R$  increases the chance of missing critical recent tokens outside the top-$k$. The performance drop is marginal, only 0.4\% from peak to lowest accuracy, demonstrating \name’s robustness to $k$. For optimal performance, we recommend setting $k$ within the range $\frac{B}{4G}$ to $\frac{B}{2G}$.

To assess the performance and robustness of our method, we perform a comprehensive hyper-parameter analysis on eight long-context tasks from LongBench, including six from Quest~\citep{tangquest} and two new additions (see Appendix). Using Llama3.1-8B-Instruct, we evaluate the effects of three key hyper-parameters: token budget, sink window size, and top-$k$, on accuracy.

These methods employ block-wise top-$k$ selection to reduce latency, but block-level memory units fail to accurately capture critical tokens, posing challenges for unit representation and inference accuracy~\cite{gao2024train}. 

as $k$ increases further, accuracy declines due to a reduction in the recent window size $R = B - S - G \times k$, where $G$ is the query group number and $S$ is the sink window size. A smaller $R$  increases the chance of missing critical recent tokens outside the top-$k$. The performance drop is marginal, only 0.4\% from peak to lowest accuracy, demonstrating \name’s robustness to $k$. For optimal performance, we recommend setting $k$ within the range $\frac{B}{4G}$ to $\frac{B}{2G}$.

% Each new token attends to the entire KV cache of length $N$, and self-attention layer with a time complexity of $O(L \times ( N \times d + d^2))$, where $d$ is the hidden dimension. In contrast, the time complexity of the feedforward network (FFN) $O(L \times 2 \times d\times d_{\text{ffn}})$. For Llama3-8B-ProLong-512k, $d_{\text{ffn}} = 3.5d$ and $d=4k$, the FFN time complexity is $O(7L\times d^2)$. As $N$ increases, the memory overhead of retrieving past keys/values becomes the primary bottleneck, making self-attention significantly slower.

% For long contexts where $N \gg 7d$, this repeated attention computation becomes a major bottleneck, significantly slowing down the generation process.


\clearpage
\newpage
\appendix
\section{Appendix}

\subsection{Attention Analysis Method}~\label{appendix:attn_analysis}

We select the Llama-3.1-8B-Instruct (128k) model as the backbone LLM for a comprehensive analysis of attention over LongBench~\citep{bai2023longbench} and InfiniteBench~\citep{zhang2024bench}. Specifically, for each task in these two benchmarks, we randomly select five examples and collect attention scores from every head and layer of the LLM. This is done for both the first token generation and token generation at another specified position.

Let $L$ and $H$ be the number of layers of LLM, the head number of attention heads per layer, respectively. Suppose that $N$ is the sequence length or KV cache size, and $k$ ($k \leq N$) is the number of top attention scores to retrain per head. Then the attention scores for a given layer $l$ ($1\leq l \leq L$) and head $h$ ($1\leq h \leq H$) can be represented as:
\begin{equation}\label{eq:attention_score}
    \mathbf{S}^{l, h} = [s_{1}^{l,h}, s_{2}^{l,h}, \cdots, s_{N}^{l,h}] \land \sum_{i=1}^{N}s_{i}^{l,h} = 1.
\end{equation}

We compute top-$k$ attentions scores $\mathbf{S}_{k}^{l,h}$ and $\mathcal{I}_{k}^{l,h}$ indexes as follows:
\begin{equation}\label{eq:topk_score}
        \mathbf{S}_{k}^{l,h} = \{s_{i}^{l,h} | i \in \mathcal{I}_{k}^{l,h}\}, \ \text{and} \  \mathcal{I}_{k}^{l,h} = \{i_1, i_2, \cdots, i_k|s_{i_1} \leq s_{i_2} \cdots \leq s_{i_k}, i_j \in \{1, 2, \cdots, N\}\}
\end{equation}

We also collect the top-$p$ token indexes (e.g., $p$ = 0.99). Let $\mathcal{I}^{l,h} = \text{argsort}_{{\text{desc}}}(\mathbf{S}^{l, h})$ represent the indices of the attention score $\mathbf{S}^{l, h}$ ordered in descending order. Then, we get the top-$p$ indexes by:
\begin{equation}
    \mathcal{I}_{p}^{l,h} = \{ i \mid i \in \mathcal{I}^{l,h}[:k], k = \min \{k^{\prime}\mid \sum_{j\in \mathcal{I}[:k^{\prime}]} s_{j}^{l, h} \geq p\} \}
\end{equation}

\xhdr{Top-$k$ Attention Score Analysis Metrics} We compute the sum of top-$k$ attention scores per head $sum_{k}^{l,h} = \sum_{i=1}^{k}\mathbf{S}_{k}^{l,h}[i]$. Then, we can get $L\times H$ sum of top-$k$ attention scores, and draw heat-map of these $L\times H$ scores. 

We calculate the sum of the top-$k$ attention scores from multiple examples drawn from diverse tasks on LongBench and InfiniteBench. All selected examples have input lengths of at least 16k tokens. The attention scores are gathered for two specific scenarios: the generation of the first token and the generation of a token at a specified position. Afterwards, we visualize the attention distribution by the following methods:
\begin{itemize}[leftmargin=2pt, parsep=0pt, topsep=0pt]
    \item \textbf{Heatmap}: A heatmap is generated for each example, where rows represent the layer index and columns represent the head index. Darker shades correspond to higher sums of the top-k attention scores.
    
    \item \textbf{Boxplot} For each layer, the sum of the top-k attention scores is aggregated across all examples. The aggregated distribution is visualized using a boxplot to show statistical summaries.

    \item \textbf{Pie Chart} The sum of the top-$k$ attention scores across all layers and examples is combined to generate a pie chart. The scores are grouped into intervals: $(0, 0.5]$, $(0.5, 0.8]$, and $(0.8, 0.9]$ and $(0.9, 1]$.
\end{itemize}


\xhdr{Top-$k$ Index Distribution Analysis Metrics}. We collect the following metrics to investigate the distribution of the top $k$ indexes.

\begin{enumerate}[leftmargin=4pt, label=(\arabic*)]
    \item \textbf{Within layer metrics}, the Jaccard similarity of top-$k$ indexes of $H$ heads, and the coverage ratio of the union of the top-$k$ indexes $\mathcal{U}_{k}^{l} = \bigcup_{i=1}^{H}\mathcal{I}_{k}^{l, i}$ to the entire context length.
    \begin{equation}
        \mathcal{J}^{l} = \frac{|\bigcap_{i=1}^{H}\mathcal{I}_{k}^{l, i}|}{|\bigcup_{i=1}^{H}\mathcal{I}_{p}^{l, i}|}, \ \text{and} \ \mathcal{R}_{c}^{l} = \frac{|\mathcal{U}_{k}^{l}|}{N},
    \end{equation}
    where $|X|$ represents the number of elements in $X$. $\mathcal{J}^{l}$ indicates the overlap ratio of top-$k$ indexes of $H$ heads in layer $l$. $\mathcal{R}_{c}^{l}$ indicates the ratio of tokens being effective or triggered by top-$k$ selection for inference in layer $l$.
    
    \item \textbf{Cross all-layer metrics}, Jaccard similarity of union of top-$k$ indexes $\mathcal{U}_{k}^{l}$ cross all $L$ layers, and the coverage ratio of the union of all union top-$k$ indexes of all layers to the entire context length.
    \begin{equation}
        \mathcal{J} = \frac{|\bigcap_{i=1}^{L}\mathcal{U}_{k}^{i}|}{|\bigcup_{i=1}^{L}\mathcal{U}_{k}^{i}|} \ \text{and} \ \mathcal{R}_{c} = \frac{|\bigcup_{i=1}^{L}\mathcal{U}_{k}^{i}|}{N}
    \end{equation}
    $\mathcal{J}$ indicates the ratio of top-$k$ tokens shared by $L$ layers. $\mathcal{R}_{c}$ indicates the ratio of tokens being effective or triggered by top-$k$ selection for inference.
    
    \item Token index frequency distribution of the top-$p$ indices across all heads and all layers. For $i$-th token ($0\leq i \leq N$), its frequency is defined as: 
    \begin{equation}
        \text{freq}_{i} = \frac{\sum_{l=1}^{L}\sum_{h=1}^{H} \mathbf{1}_{ i \in \mathcal{I}_{p}^{l, h}}}{L \times H}.
    \end{equation}
\end{enumerate}

\subsection{StreamLLM with Relative and Absolute Positions}\label{append:stream_position}

\begin{figure}[!h] % "t" places the figure at the top of the page
    \centering
    \includegraphics[width=0.8\textwidth]{figures/StreamLLMPosition.pdf} % Adjust width as needed
    \caption{Implementation of Absolute and Relative Positioning in StreamLLM. Relative position assigns indices within StreamLLM’s sliding window, dynamically shifting as the window moves to maintain a bounded range. In contrast, absolute position assigns a fixed index to each token based on its original sequence, increasing continuously as new tokens are added.}
    \label{fig:streamLLM_position} % Label for referencing the figure
\end{figure}


\subsection{Implementation Details of \name with LLMs}

\xhdr{Hyper-parameter settings} For our method \name, suppose that the token budget is $B$ and the query group number is $G = h_{q} / h_{v}$ where $h_{q}$ and $h_{kv}$ are the query head number and ke/value head number, respectively, we set the sink window as $B/4$, and $k$ = $\frac{B}{2G}$, and the recent window size as $B/4$. For Llama3.1-8B-Instruct and Llama-3-8B-ProLong-512k-Instruct, we set $B$ = 8192, and thus sink window size = 2048 and $k$ = 1024, the local window size = 2048. For Qwen2.5, since the query group number is 7, we set $B$ = 8192, thus sink window size = 2048, $k$ = 512 and the local window size = 8192 - 2048 - 7 $\cdot$ 512 = 2560. For other baselines, we set the same token budget $B$ 8192. Absolute positioning is applied in \name to the reduced KV cache to maintain token order.

\xhdr{Task names for Hyper-parameter analysis} We use the following eight LongBench tasks for hyper-parameter analysis, as in~\citep{tangquest}: ``gov-report", ``multifieldqa-en", ``narrativeqa", ``passage-retrieval-en", ``qasper", ``repobench-p", ``hotpotqa", and ``triviaqa".


\subsection{Experimental Results over InfiniteBench}

\begin{table}[h!]
\centering
\caption{Comparison of KV Cache Eviction Methods on InfiniteBench with Different LLMs}
\label{tab:infinite_acc}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
Method &  Code.Debug  & Choice.En & Math.Find & Number & PassKey & QA.CH & Book.Sum & QA.EN & Diag.EN & Average \\ \midrule
\multicolumn{11}{c}{Llama3.1-8B-Instruct (128k)} \\
\midrule
FullAttention      & 22.59 & 61.57 & 25.14 & 99.49 & 100.0 & 34.53 & 16.82 & 35.44 & 22.5 & 46.45 \\  
StreamLLM$_{HF}$      & 22.84 & 62.88 & 25.14 & 3.73 & 6.78 & 27.71 & 13.8 & 31.26 & 17.0 & 23.46     \\
StreamLLM$_{R}$     & 22.59 & 60.7 & 32.57 & 6.61 & 6.78 & 25.33 & 16.49 & 30.35 & 14.5 & 23.99 \\
StreamLLM$_{Abs}$   &   22.59 & 62.88 & 24.57 & 5.59 & 6.78 & 26.71 & 16.0 & 31.05 & 14.5 & 23.41 \\   
% Quest & x     & x     & x     & x     & x     & x     & x     & x     & x  & x  \\
% InfLLM & 22.59& 43.23& 32.57& 100& 100& x     & x     & x     & x  & x  \\
\name (ours) & 22.59 & 62.88 & 26.0 & 94.24 & 100.0 & 30.51 & 16.47 & 33.01 & 20.5 & 45.13 \\
\midrule
\multicolumn{11}{c}{Llama-3-8B-ProLong-512k-Instruct}\\
\midrule
FullAttention   &  38.83 & 63.76 & 20.86 & 100.0 & 100.0 & 28.37 & 8.48 & 33.36 & 10.5 & 44.91 \\ 
\midrule
StreamLLM$_{HF}$    & 39.85 & 64.19 & 20.86 & 5.08 & 6.78 & 23.8 & 7.69 & 28.2 & 9.0 & 22.83 \\
StreamLLM$_{R}$    & 36.55 & 63.76 & 21.43 & 6.78 & 6.78 & 22.97 & 9.61 & 28.19 & 9.5 & 22.84 \\
StreamLLM$_{Abs}$    & 36.55 & 63.76 & 22.0 & 6.78 & 6.78 & 22.54 & 9.93 & 27.58 & 10.0 & 22.88 \\  
% Quest & x     & x     & x     & x     & x     & x     & x     & x     & x  & x  \\
% InfLLM & 27.66& 43.67& 18.86& 99.83& 95.25& x     & x     & x     & x  & x  \\
\name (ours) & 36.04 & 63.76 & 21.43 & 86.78 & 100.0 & 26.41 & 8.24 & 32.77 & 10.5 & 42.88 \\
\midrule
\multicolumn{11}{c}{Qwen2.5-7B-Instruct (128k)}\\
\midrule
FullAttention      & 33.5 & 49.78 & 33.43 & 94.58 & 96.44 & 28.09 & 12.33 & 15.96 & 11.5 & 41.73 (26.37) \\
\midrule
StreamLLM$_{HF}$   & 30.46 & 51.97 & 28.0 & 0.51 & 5.08 & 10.35 & 10.98 & 5.72 & 12.5 & 17.29 (21.43) \\
StreamLLM$_{R}$     & 27.41 & 51.09 & 39.43 & 6.78 & 6.78 & 22.79 & 14.97 & 14.77 & 11.0 & 21.67 (25.92) \\
StreamLLM$_{Abs}$    & 31.47 & 48.03 & 28.57 & 5.08 & 5.08 & 22.64 & 14.11 & 13.45 & 9.5 & 19.77 (23.97) \\   
% Quest & x     & x     & x     & x     & x     & x     & x     & x     & x  & x  \\
% InfLLM & 22.59& 51.97& 38.57& 95.25& 93.9& x     & x     & x     & x  & x  \\
\name (ours) & 32.23 & 48.47 & 34.86 & 5.25 & 47.29 & 27.66 & 12.76 & 15.58 & 11.0 & 26.12 (26.08) \\
 \bottomrule
 \multicolumn{11}{l}{Note: For Qwen2.5-7B-Instruct, we also report average accuracy (in parentheses) excluding the ``Number" and ``PassKey" retrieval tasks.}\\
% Add more rows as needed
\end{tabular}%
}
\end{table}
%++++++++++++++++

Table~\ref{tab:infinite_acc} compares the accuracy of Llama-3-based and Qwen2.5 models on InfiniteBench. The results show that:
\begin{itemize}[leftmargin=2pt, parsep=0pt, topsep=0pt]
    \item \name achieves accuracy comparable to full attention in long-context LLaMA models, including LLaMA3.1-8B-Instruct and LLaMA3-8B-ProLong-512k-Instruct. Unlike traditional methods, it selects key tokens in a single pass using the last input token’s attention scores, eliminating per-token selection during generation. For Qwen2.5-7B-Instruct, \name matches full attention in most tasks, except for two retrieval benchmarks (Number and PassKey), while still outperforming StreamLLM. This highlights LLMs’ ability to naturally prioritize critical tokens for effective response generation.  
    
    \item StreamLLM’s static sparse KV selection leads to suboptimal accuracy in long-context LLMs by discarding essential information from the middle of the input sequence. However, our implementation outperforms the official Hugging Face (HF) version, achieving significantly better performance with Qwen2.5-7B-Instruction and slightly higher average accuracy with Llama3.1-8B-Instruct. These findings underscore the importance of precise implementation in evaluating StreamLLM, especially for models sensitive to token-relative positioning, consistent with the results in LongBench (Table~\ref{tab:long_bench}).
\end{itemize}


Fig.~\ref{fig:framework} illustrates the framework of our proposed \name for efficient long-context inference. In this work, we focus on accelerating token generation, assuming the pre-filling stage is complete.



\subsection{Overall Framework}


Long-context Large Language Models (LLMs) are vital for processing complex inputs and have diverse applications, including summarization, multi-hop reasoning, question answering, code understanding, personalized chatbots, recommendation systems, and in-context learning~\citep{zhou2024survey,li2024survey,gpt4o,team2024gemini}. Despite their significant benefits, long-context LLMs face substantial challenges, primarily stemming from increased computational demands. Supporting long-context inference is particularly expensive due to two key factors: the high memory requirements of the KV (Key-Value) cache and the significant latency involved in attention computation~\citep{li2024survey}. The latency of attention computation, which dominates the inference process, scales proportionally with the size of the KV cache. This makes efficient management of memory and computational resources critical for enabling the practical use of long-context LLMs in real-world applications. Addressing these challenges is essential for unlocking the full potential of long-context LLMs.

In contrast, dynamic sparsity-based KV cache methods assume that the sparse patterns are context-dependent and adaptively select representative tokens for each new token generation, often achieving better performance than static sparsity approaches. However, they are computationally intensive and rely on carefully tuned hyperparameters, such as the chunk/block size in InfLLM~\citep{xiao2024infllm} and Quest~\citep{tangquest}, or complex ANN (Approximate Nearest Neighbors) index construction in RetrievalAttention~\citep{liu2024retrievalattention}. These methods do not reduce memory usage because the entire KV cache must be retained as a candidate pool at each generation step. Additionally, all block-level KV caches must also reside in GPU memory, further increasing memory demands. Although offloading the KV cache to the CPU can reduce GPU memory usage, it introduces significant overhead due to the latency of retrieving sparse KV pairs during decoding~\citep{sun2024shadowkv}. Consequently, dynamic methods require sophisticated designs to balance computational efficiency and communication overhead, often involving tightly integrated CPU-GPU computations or communication strategies, which increases implementation complexity~\citep{xiao2024infllm,lee2024infinigen,he2024fastdecode,liu2024retrievalattention}.


In this paper, we tackle the challenges of efficient long-context inference in LLMs by leveraging the observation that LLMs inherently possess the ability to identify the critical information after the pre-filling stage. Based on the sparsity of attention scores over long context inference, that the attention scores exhibit head-level sparsity and effectively highlight the importance of tokens within the context. This insight forms the basis for optimizing KV cache compression at the head level. Building on this analysis, we introduce a novel method, \textbf{\underline{S}elf-\underline{A}ttention \underline{G}uided \underline{E}viction for KV Cache} (\name) (See Fig.\ref{fig:framework}), which uses attention scores to guide the eviction process, significantly improving the efficiency of long-context inference.

Our method, \name, employs a single-pass token-level KV cache selection strategy, compressing the KV cache once after the pre-filling stage using attention scores (Please see Fig.~\ref{fig:framework}). 
Only the compressed KV cache is retained in memory, eliminating the need for further repetitive KV selection during token generation, as required by block-level dynamic KV selection methods. This significantly reduces computational overhead while preserving essential information for inference. The compressed KV cache retains only the most relevant information, facilitating both efficient and accurate inference. \name leverages the efficiency of static sparse patterns—benefiting from their single-pass nature and fixed structure during subsequent generations—while integrating the adaptability of dynamic selection methods, allowing KV cache selection to be context-dependent. This combination enables \name to achieve superior efficiency while maintaining or even improving performance compared to existing dynamic block-level KV cache selection approaches. This is substantiated by our extensive experiments conducted across various long-context LLMs and benchmarks. Furthermore, our method achieves nearly 4× and 2× higher memory efficiency and improved accuracy compared to the static KV eviction method StreamLLM and the dynamic block-level KV eviction method Quest, respectively. This simple yet effective solution accelerates long-context inference while offering ease of integration, providing a promising direction for addressing the challenges of long-context LLM inference.

Considering a long input text sequence $s = [t_{i}]_{i=1}^{N}$ of length $N$, consisting of a context followed by a query. After the prefilling step, the full key-value vectors (i.e., KV cache) for layer $l$ are obtained as $\mathbf{P}^{l} = [(\mathbf{k}_i^{l}, \mathbf{v}_i^{l})]_{i=1}^{N}$. As shown in Fig.~\ref{fig:framework}, the proposed method involves the following steps.

For a comprehensive evaluation, we compare our method against the following baselines: 1) \textbf{Full-Attention Models}: standard models using full attention. 2) \textbf{Hugging Face StreamLLM}~\citep{xiaoefficient}: The official StreamLLM implementation by Hugging Face. 3) \textbf{Our Implementation of StreamLLM}: To address position information conflicts in the Hugging Face implementation~\citep{xiaoefficient} (see \url{https://github.com/huggingface/transformers/issues/35350}), we introduce two variants: $\text{StreamLLM}R$, which stores the pre-RoPE KV cache and applies relative positional encoding during attention, and $\text{StreamLLM}{Abs}$, which applies absolute positional encoding~\citep{su2024roformer}. 4) \textbf{Quest}~\citep{tangquest}: a dynamic approach using block-wise top-$k$ selection for each token generation. and 5) \textbf{InfLLM}~\citep{xiao2024infllm}: another dynamic method that integrates sink tokens, recent tokens, and block-wise top-$k$ selection at each generation step.

\name achieves accuracy comparable to full attention by leveraging self-attention-guided KV cache selection after the pre-filling stage. Notably, our approach uses a single-pass selection process based on the attention scores of the last token in the input sequence, rather than performing this selection for every token generation. This demonstrates that LLMs inherently identify and prioritize critical tokens needed to answer a given question effectively.

    StreamLLM’s static sparse pattern-based KV selection results in suboptimal accuracy for long-context LLMs since it discards essential information from the middle of the input sequence. Notably, our StreamLLM implementation outperforms the official Hugging Face (HF) version, achieving significantly better performance with Qwen2.5-7B-Instruction and slightly higher average accuracy with Llama3.1-8B-Instruct. This improvement likely results from a flaw in the HF implementation, where the RoPE rotation operation fails to correctly update key cache positions, increasing relative distances between adjacent tokens. As documented in~\citet{hf_github_bug}, this issue particularly affects Qwen2.5’s sensitivity to positional encoding. In contrast, our implementation properly scales relative distances, ensuring more stable performance. These findings highlight the critical role of precise implementation in evaluating StreamLLM, particularly for models sensitive to token-relative positioning.

Dynamic sparse pattern-based KV selection methods, such as InfLLM and Quest, retrieve relevant blocks at each generation step but underperform compared to \name. Their lower accuracy stems from block-wise top-$k$ selection, which relies on representative vectors from block-wise pooling, weakening important token identification~\citep{liu2024retrievalattention,tangquest}. While these methods reduce latency by operating at the block level, they struggle to capture critical tokens accurately, leading to suboptimal unit representation and inference accuracy~\citep{gao2024train}. In contrast, \name employs token-level selection, closely approximating full attention and achieving higher accuracy than dynamic top-$k$ KV cache block selection. This underscores the importance of precise token selection in maintaining high inference accuracy while reducing KV cache size.


We introduce \name, an efficient KV cache eviction method for long-context LLM inference. By leveraging attention sparsity, \name compresses the KV cache after the prefilling stage for direct use in generation. Our experiments demonstrate that \name achieves inference speeds comparable to static sparse methods while maintaining accuracy close to full attention. Notably, it provides \textit{4x higher memory efficiency} and \textit{improved accuracy} over the static KV cache eviction method StreamLLM, and \textit{2x higher memory efficiency} with \textit{better accuracy} than the dynamic KV cache eviction method Quest. Moreover, \name seamlessly integrates with popular LLM frameworks, including Hugging Face Transformers, Meta’s LLaMA, and Alibaba’s Qwen, ensuring broad applicability in existing pipelines.
